Automatic Generation of Benchmarks and Reliable LLM Judgment for Code Tasks

LLMs can be used in a variety of code related tasks such as translating from one programming language to another, implementing natural language requirements and code summarization. Artifacts generated by state of the art LLM technology are expected to be useful in the sense that a user will be able to use the LLM generated artifact after a small number of easy modifications. Quantifying this vague notion is challenging and it is thus hard to determine the quality of code related LLM solutions. We refer to evaluation of LLM solutions using LLM judgment as "LLM as a Judge", or LaaJ for short. In this work we introduce a methodology to generate and evaluate LaaJ implementations, utilizing an automatically generated benchmark. The purpose of the benchmark is two fold, namely, it is used both to develop and validate the LaaJs and to validate and test the LLM code related solution using the LaaJs. To that end, we developed an automated benchmark generation engine, which generates code in multiple programming languages for multiple code related tasks and which serves as the input for LaaJ evaluation. We utilize a graph representation, G, of the potential code related generations. The graph vertices are generated artifacts and edges represent possible generations, e.g., the generation of a Java program from its natural language requirements. Utilizing a chain of LLM agents and G we generate code related artifacts. Using cycles in G we formulate expectations on the generated artifacts. Taking advantage of these formulated expectations enables the development and testing of reliable LLM judgement for usefulness of the artifacts generated by the solution. Our approach enables the creation of high quality code task solutions.

==> relatedWork.tex <==
\section{Related work}

Generated code evaluation could rely on functional correctness, evaluated by executing code against robust tests \cite{Chen2021Evaluating}, but, this is feasible only for simple code related generation and translation tasks.  In addition, code development use cases and task such as code completion does not assume that the code even compiles let alone run.  Finally,  other code related tasks such as sumerization do not lend themselves to runtime evaluation.
Thus, a holistic approach to evaluation of code related tasks usefulness can not rely solely on runtime evaluation. 

Automatic static evaluation metrics are used to evaluate code related tasks. \emph{Reference-based metrics} compare generated code to reference code. BLEU \cite{Papineni2002BleuAM}, ROUGE-L \cite{Lin2004ROUGEAP}, and chrF++ \cite{Popovic2017chrFWH} treat code as text, focusing on n-gram statistics. CodeBLEU \cite{ren2020codebleu} incorporates code structure, while CodeBERTScore \cite{zhou-etal-2023-codebertscore} leverages semantic information in the embedding space. \emph{reference-less metrics} have been explored, such as ICE-Score \cite{zhuo2024icescore}, which employs the concept of LLMaaJ, utilizing the advanced understanding of both code and natural language by LLMs.  

However, these metrics often fail to capture the functional usefulness of generated code, either underestimating the variety of correct solutions or overestimating the advanced understanding of LLMs. Research has shown that BLEU scores weakly correlate with human judgment in code-related tasks \cite{8813269}, and no static evaluation metric consistently aligns with human preferences for code correctness and quality \cite{evtikhiev2023bleu}. 

%TBC 
%Add to related work  as it uses the reverse model idea 
%The Llama paper link:
%https://ai.meta.com/research/publications/the-llama-3-herd-of-models/

%In \cite{weyssow2024codeultrafeedbackllmasajudgedatasetaligning} LaaJ is used to tune code generation to a particular programming style (\href{https://arxiv.org/abs/2403.09032}{link}).  

%In \cite{shi2024naturallanguageoutlinescode} (see \href{file:///C:/Users/289500756/Downloads/Natural%20Language%20Outlines%20for%20Code%20-%20Literate%20Programming%20in%20the%20LLM%20Era%20(1).pdf}{link}) a paradigm of developing a program using natural language by utilizing LLM capabilities.  In the context of testing and generation of long programs for self consistency benchmarks this paradigm may be applied. 


==> tuning.tex <==
\section{Tuning the LLM judgment}

To tune the LLM judgment regardless of the way the judgment is constructed one needs to measure the quality of the judgement.  To achieve that two approaches are detailed below.  The first approach  contrast the LLM judgment with human judgment and the second consider consistency requirements over the LLM judgment. 

\subsection{Human judgement consistency}
\label{humanConsistency}

Typical human judgment ranking should be treated as an ordinal measure (see \href{(https://www.questionpro.com/blog/nominal-ordinal-interval-ratio/}{link}) or a utility that expresses human preference.  Thus, the absolute numbers and the distances between them such as the difference $|i-j|$ between two ranking scores, $i, j$ does not capture a lot of information about the human preference, i.e., how big $|i-j$ is assuming $i>j$ does not reflect to what extend $i$ is preferred over $j$.

\begin{example}
For example, 
human scores for 4 samples are:  $A=4, B=5, C=6, D=7$
LLM judge, $LLM_1$, scores for them: $A=4, B=5, C=7, D=6$
while LLM judge $LLM_2$ scores for them: $A=3, B=4, C=5, E=6$
Aiming for the best human-score match gives $|4-4|+|5-5|+|6-7|+|7-6|=2$ score to $LLM_1$ and $|3-4|+|4-5|+|5-6|+|6-7|=4$ to $LLM_2$.  We determine that $LLM_1$ is better, while $LLM_2$ ownered the order of the human judgment!
Particularly, $LLM_1$ mistakenly thinks $C$ is better than $D$, while $LLM_2$ is matching the human judgment on $C$ and $D$ and is a better choice as a proxy for the human judgment.
\end{example}

A general way to think about the human ranking of the benchmark $B$ is as an ordering over the elements of $B$.  Given two data points $x, y \in B$ the human judgment dictates if the "golden" generation $g(x)$ is preferred to $g(y)$ by giving $g(x)$ an higher rank.  We utilize this observation to test the LLM judgement as follows.  Given that the LLM-judge ranks $g(x)$ and $g(y)$ we are interested in whether or not it ranked it in the same way as the order given by the human judgment (see also \href{https://en.wikipedia.org/wiki/Kendall_rank_correlation_coefficient}{Kenfal rank correlation}.).  We thus have the indicator function $I(x, y)$ that is $1$ if the LLM judge agrees with the order determined by the human and $0$ otherwise.  To estimate the quality of the LLM-judge we randomly sample n=20 to n=30 pairs of data point $x, y \in B$ and obtain a sample $S \subseteq B \times B$.  We then calculate the average $\frac{\sum_{(x, y) \in S} I(x, y)}{n}$.  See implementation here \href{https://colab.research.google.com/drive/17scwgI9k-uC3-fKAt_j32I46iyTE0tSO?usp=sharing}{link}.

Previous work on perturbations of the code has attempted to assess the robustness of LLM code related tasks \cite{wang-etal-2023-recode}.  Sometimes the golden results $g(x), g(y)$ can be perturbed in such a way that the meaning is preserved.  In those cases we expect the LLM-judge to provide the same ordering as the human originally did regardless of the perturbations.   Introducing perturbations in such a way may result in a stronger test of the LLM judgment.  Assume that $P(g(x))$ is the set of perturbations of $g(x)$ and similarly $P(g(y))$ is the set of perturbations of $g(y)$ we then obtain an LLM judgment for each pair $a \in P(g(x)), b \in P(g(y))$.  The percentage of agreement of the LLM judgement with the golden judgment is then the new score  $I(x, y)$. 

In the special case in which the LLM judgment is done through ranking we will have that the ranks of $a \in P(g(x))$ by the LLM judge is expected to be equal to the rank of $g(X)$.  Similarly, for $g(Y)$.

\subsection{LLM internal consistency}

The LLM represents a preference that should proxy human preference.   A natural requirement for preference consistency is transitivity.  Given three data points $x, y, z \in B$ such that the LLM judges that the generation $g(x)$ is better than $g(y)$, $g(x) >_{LLM} g(y)$ and also that $g(y)$ is better than $g(z)$, $g(y) >_{LLM} g(z)$ we would expect to see that $g(x) >_{LLM} g(z)$.  We thus define an indicator function $I_t(x, y, z)$ that is $1$ if the LLM judgment was transitive for $(x, y, z)$ and $0$ otherwise.  Sampling $n=20$ to $30$ triples $x, y, z$ from $B$ we get a set of triples $S \subseteq B \times B \times B$. We can then obtain an average score for transitivity $\frac{\sum_{(x, y, z) \in S} I(x, y, z)}{n}$. See implementation here \href{https://colab.research.google.com/drive/17scwgI9k-uC3-fKAt_j32I46iyTE0tSO?usp=sharing}{link}.

Internal consistency can be implemented in ways that are more general than transitivity.  For example, one could ask a LLM to judge if the translation from one language to another is correct and also ask to determine if the source and translated programs produce the same output.   We expect that the judgments should agree.  Thus, we can use the comparison of the two judgements to determine if the LLM is able to consistently judge the generation of the target code.  

Another more generic example of this internal consistency paradigm is as follows.  Given a code sample $S$ ask an LLM to rank the translations, $g(x), x \in S$ by $r(g(x))$ and also ask an LLM to determine if $g(x)$ is better than $g(y)$ for all $x, y \in S$.  We then expect that if $r(g(x)) > r(g(y))$ then the LLM will judge $g(x)$ to be better than $g(y)$.  

\subsection{Using LLM judgment to bootstrap human labeling}

When the token limitation is not hit LLM judgment can be utilized to bootstrap ranking of a new model, $LLM_N$, assuming the results of a previous model generation, $LLM_P$, were ranked by a human.    

Assuming that we have given $n$ code samples, $S_1, \ldots, S_n$,  In addition, we are given $n$ artifacts, e.g., summaries, $LLM_P(S_1), \ldots, LLM_P(S_n)$ and their associated human ranking $r(LLM_P(S_1)), \ldots, r(LLM_P(S_n))$ we proceed as follows. 

\begin{enumerate}
    \item Using a $LaaJ$ to rank the artifacts produced by the new,$LLM_N$.  The $LaaJ$ ranking uses the previous ranking of $LLM_P$ results.  We thus obtain $n$ new ranks, 
    
    $LaaJ(LLM_N(S_1), LLM_P(S_1), r(LLM_P(S_1))), \ldots, LaaJ(LLM_N(S_n), LLM_P(S_n), r(LLM_P(S_n))) $   
    \item We sample 20-30 points from $S_1, \ldots, S_n$ and rank them by humans.  If the ranking of the humans agrees with the ranking of the $LaaJ$ we accept the ranking of the $LaaJ$ as the golden truth and proceed as before.   To check the agreement of the $LaaJ$ ranking and the the human ranking we apply the same approach as in \ref{humanConsistency}.
\end{enumerate}

\subsection{Analyzing different types of errors}

A given $LLM$ model, $M$, is tested on a benchmark, $B$, using $n$ $LLM$ judges that identify $n$ types of errors $N = \{1, \ldots, n\}$.  It is found out that $M$ made $m_1 > \ldots > m_n$ mistakes where $m_i$ is the number of errors of type $i$ made in $B$.  
We also rank the errors types by $w(m_1) > \ldots w(m_n)$ where $w(m_i)$ indicates how severe the error of type $i$ is.  
We thus have that the measure of weighted error that $M$ performed is $C(M) = \sum_{i \in N} w(m_i) \times m_i$.  

If we are given another, possible golden model, to compare to we apply the  \href{https://en.wikipedia.org/wiki/Jaccard_index}{weighted Jaccard similarity}.  In details given that the counts of the reference model, $M_r$, on $B$ are $m^r_1 > \ldots > m^r_n$ we get the error measure of $J_w(M, M_r) =  \frac{\sum_{i \in N} min(m^r_i, m_i)}{\sum_{i \in N} max(m^r_i, m_i)}$\footnote{Note that $1 -J_w(M, M_r)$ is a distance.}. 
